Cross-document Event Identity via Dense Annotation

In this paper, we study the identity of textual events from different documents. While the complex nature of event identity is previously studied (Hovy et al., 2013), the case of events across documents is unclear. Prior work on cross-document event coreference has two main drawbacks. First, they restrict the annotations to a limited set of event types. Second, they insufficiently tackle the concept of event identity. Such annotation setup reduces the pool of event mentions and prevents one from considering the possibility of quasi-identity relations. We propose a dense annotation approach for cross-document event coreference, comprising a rich source of event mentions and a dense annotation effort between related document pairs. To this end, we design a new annotation workflow with careful quality control and an easy-to-use annotation interface. In addition to the links, we further collect overlapping event contexts, including time, location, and participants, to shed some light on the relation between identity decisions and context. We present an open-access dataset for cross-document event coreference, CDEC-WN, collected from English Wikinews and open-source our annotation toolkit to encourage further research on cross-document tasks.

==> images/non_transitivity_example.tex <==
\begin{figure}[t]
\centering
\resizebox{0.4\textwidth}{!}{
\begin{tikzpicture}[
rectnode/.style={rectangle, thick, align=center, minimum size=2.5cm},
]
%Nodes
\node[rectnode] (1c) [text width=6cm] {That quake was followed by as many as 60 \textbf{aftershocks} for at least a week, with some ranging as high as magnitude 7.8.};
\node[rectnode] (1a) [below right=1cm and -2.75cm of 1c,text width=2.5cm] {It was first reported to be a 7.3 \textbf{aftershock}.};
\node[rectnode] (1b) [below left=1cm and -2.75cm of 1c,text width=3.5cm] {Some smaller \textbf{aftershocks} with magnitudes between 5.2 and 5.7 were also reported in the region.};

%Lines
\draw[<->,draw=red,very thick] (1a.west) -- (1b.east) node[midway,below] {\xmark};
\draw[<->,draw=blue,very thick] (1a.north) -- ([xshift=0.1cm]1c.south) node[midway,above right] {\cmark};
\draw[<->,draw=blue,very thick] (1b.north) -- ([xshift=-0.1cm]1c.south) node[midway,above left] {\cmark};

\end{tikzpicture}}

\caption{An illustration of the quasi-identity nature of events. The mention `[60] aftershocks' is only partially identical to the two mentions `[smaller] aftershocks' and `[7.3] aftershock', thus leading to two partial coreference links (\cmark). Interestingly, the third mention pair is non-coreferential (\xmark), indicating that partial coreference need not satisfy the transitivity property.}
\label{fig:non_transitivity_example}
\end{figure}

==> tables/intro_example.tex <==
\begin{table*}[ht]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}l@{ \ }p{\textwidth}@{}}
    \toprule
    1a & It was first reported to be a 7.3 \textbf{aftershock}. \\
    1b & Some smaller \textbf{aftershocks} with magnitudes between 5.2 and 5.7 were also reported in the region. \\
    1c & That quake was followed by as many as 60 \textbf{aftershocks} for at least a week, with some ranging as high as magnitude 7.8. \\
    \midrule
    2a & Tropical \textbf{storm} Richard is nearing hurricane strength with winds of 70 mph (115 kph) as it lashes Honduras with heavy rains \\
    2b & \textbf{Hurricane} Richard made landfall in Belize about 20 mi (35 km) south-southeast of Belize City with winds of 90 mph (150 kph) at approximately 6:45 local time (0045 UTC) according to the National Hurricane Center (NHC) \\
    \bottomrule
    \end{tabular}}
    \caption{An illustration of quasi-identity of events in cross-document event coreference. Example 1 illustrates the issue of coreference clustering when mentions are only partially identical. Examples 2 showcases the spatiotemporal continuity of the event \textit{Richard}. While the two mentions (storm, hurricane) depict slightly different realizations of the event \textit{Richard}, they share a common identity. }
    \label{tab:intro_example}
\end{table*}
